JWST NIRSpec spectroscopy of the triply-lensed $z = 10.17$ galaxy MACS0647$-$JD

We present JWST/NIRSpec prism spectroscopy of MACS0647-JD, the triply-lensed $z \sim 11$ candidate discovered in HST imaging and spatially resolved by JWST imaging into two components A and B. Spectroscopy of component A yields a spectroscopic redshift $z=10.17$ based on 7 detected emission lines: CIII] $\lambda\lambda$1907,1909, [OII] $\lambda$3727, [NeIII] $\lambda$3869, [NeIII] $\lambda$3968, H$\delta$ $\lambda$4101, H$\gamma$ $\lambda$4340, and [OIII] $\lambda$4363. These are the second-most distant detections of these emission lines to date, in a galaxy observed just 460 million years after the Big Bang. Based on observed and extrapolated line flux ratios we derive a gas-phase metallicity $Z =$ log(O/H) = $7.5 - 8.0$, or $(0.06 - 0.2)$ $Z_\odot$, ionization parameter log($U$) $\sim -1.9\pm0.2$, and an ionizing photon production efficiency ${\rm log}(\xi_{\rm ion})=25.2\pm0.2\,$erg$^{-1}$ Hz. The spectrum has a softened Lyman-$\alpha$ break, evidence for a strong Ly$\alpha$ damping wing, suggesting that MACS0647-JD was unable to ionize its surroundings beyond its immediate vicinity ($R_{\text{HII}} \ll 1$ pMpc). The Ly$\alpha$ damping wing also suppresses the F150W photometry, explaining the slightly overestimated photometric redshift $z = 10.6 \pm 0.3$. MACS0647-JD has a stellar mass log($M/M_\odot$) = $8.1 \pm 0.3$, including $\sim$ 6$\times 10^7 M_\odot$ in component A, most of which formed recently (within $\sim$ 20 Myr) with a star formation rate $2\pm1 M_\odot$ / yr, all within an effective radius $70\pm24\,$pc. The smaller component B ($r \sim 20$) pc is likely older ($\sim$100 Myr) with more dust ($A_V \sim 0.1$ mag), as found previously. Spectroscopy of a fainter companion galaxy C separated by a distance of \about\ 3$\,$kpc reveals a Lyman break consistent with $z = 10.17$. MACS0647-JD is likely the most distant galaxy merger known.

==> line_flux_b.tex <==
% Filters
\begin{deluxetable*}{lccrcr}
\tablecaption{\label{tab:lines}Estimated line fluxes
}
\tablewidth{\columnwidth}
\tablehead{
\colhead{MACS0647--JD} &
\colhead{\CIIId} &
\colhead{\OII} &
\colhead{\NeIII} &
\colhead{\Hdelta} &
\colhead{\Hgamma}
}
\startdata
Rest wavelength ($\rm \AA$)
& 1907 \& 1909
& 3727 
& 3869 
& 4101 
& 4340 \\
Observed wavelength ($\rm \mu m$)
& 2.13
& 4.16
& 4.32 
& 4.58 
& 4.85 \\
Equivalent width
& 
& 
& 
& 
& \\
\hline
\hline
\multicolumn{6}{c}{Obs 21 JD2}\\
\hline 
Line fluxes ($10^{-20}\,$erg/s/cm$^2$) 
&  $131.6\pm22.5$
&  $27.1\pm6.2$ 
& $48.2\pm5.9$
& $28.7\p6.1$ 
& $70.8\pm5.7$ \\
SNR
& $5.8$
& $4.4$ 
& $8.2$
& $5.9$ 
& $12.4$\\
\hline
\hline
\multicolumn{6}{c}{Obs 23 JD1}\\
\hline 
Line fluxes ($10^{-20}\,$erg/s/cm$^2$) 
&  $101.8\pm22.9$
&  $15.8\pm6.3$ 
& $39.9\pm6.4$
& $11.9\pm6.6$ 
& $52.1\pm6.7$ \\
SNR
& $4.4$
& $2.5$ 
& $6.2$
& $1.8$ 
& $7.8$\\
\hline
\hline
\multicolumn{6}{c}{Obs 23 JD2}\\
\hline 
Line fluxes ($10^{-20}\,$erg/s/cm$^2$) 
&  $137.4\pm26.4$
&  $27.2\pm7.0$ 
& $35.5\pm6.3$
& $20.7\pm7.1$ 
& $43.5\pm7.5$ \\
SNR
& $5.2$
& $3.9$ 
& $5.6$
& $2.9$ 
& $5.8$\\
\hline
\hline
\multicolumn{6}{c}{Stack}\\
\hline 
Line fluxes ($10^{-20}\,$erg/s/cm$^2$) 
&  $314.0\pm54.9$
&  $41.7\pm4.7$ 
& $40.8\pm5.6$
& $39.6\pm6.5$ 
& $74.4\pm9.6$ \\
SNR
& $5.7$
& $8.9$ 
& $7.3$
& $6.1$ 
& $7.7$\\
\enddata
\tablenotetext{}{
{{\textbf{Note}. 
}}}%\tablenotetext{a}{Mass-weighted}
%\tablecomments{
%\cite{Hopkins10} find maximum stellar mass density $10^{11} M_\odot$ kpc$^{-2}$ = $10^5 M_\odot$ pc$^{-2}$.
%We're just below that.
%SMGs $> 1000 M_\odot$ yr$^{-1}$ kpc$^{-2}$. We're also below that.
%}
\end{deluxetable*}
% https://docs.google.com/spreadsheets/d/1k5Xgf7vtZjnpvPa5rycbFL_WlGYhXsqBX5VMnrCTFos


==> line_flux_rescaled.tex <==
% Filters
\begin{deluxetable*}{lccrcc}
\tablecaption{\label{tab:lines}Measured emission line fluxes
}
\tablewidth{\columnwidth}
\tablehead{
\colhead{Emission Lines} &
\colhead{Rest wavelength} &
\colhead{Observed wavelength} &
\colhead{Line fluxes\supa\ } &
\colhead{SNR} &
\colhead{Equivalent width}
\vspace{-0.07in}\\
\colhead{} &
\colhead{$\rm \AA$}  &
\colhead{$\rm \mu m$} &
\colhead{$10^{-20}\,$erg/s/cm$^2$} &
\colhead{} &
\colhead{$\rm \AA$} 
}
\startdata
%\CIIIdw
\CIIId
& 1907, 1909
& 2.13
& $314.0\pm54.9$
& $5.7$
&  14.2\\
%\OIIw
\OII
& 3726, 3729
& 4.16
& $41.7\pm4.7$ 
& $8.9$ 
&  13.1\\
%\NeIIIw 
\NeIII
& 3869 
& 4.32 
& $76.0\pm5.5$
& $13.8$
&  25.2\\
\NeIII%\,\lambda 3968 
& 3968
& 4.43
& $40.8\pm5.6$
& $7.3$
& 14.8\\
\Hdelta
& 4101 
& 4.58 
& $39.6\pm6.5$
& $6.1$ 
&  17.1\\
\Hgamma
& 4340
& 4.85
& $74.4\pm9.6$
& $7.7$
& 41.8\\
\OIII%\,\lambda4363
& 4363 
& 4.87
& $25.0\pm5.6$ 
& $4.4$ 
&  14.4\\
HeI%\,\lambda4473
& 4473 
& 5.00
& $24.3\pm8.8$ 
& $2.8$ 
& 15.7 \\
\enddata
\tablenotetext{}{
{{\textbf{Note}. 
}}}
\tablenotetext{a}{As observed in the stack of 4 observations with total magnification \about 27}
%\tablecomments{
%\cite{Hopkins10} find maximum stellar mass density $10^{11} M_\odot$ kpc$^{-2}$ = $10^5 M_\odot$ pc$^{-2}$.
%We're just below that.
%SMGs $> 1000 M_\odot$ yr$^{-1}$ kpc$^{-2}$. We're also below that.
%}
\end{deluxetable*}
% https://docs.google.com/spreadsheets/d/1k5Xgf7vtZjnpvPa5rycbFL_WlGYhXsqBX5VMnrCTFos


==> photometry_bu.tex <==
% Filters
\begin{deluxetable*}{lllcccr}
\tablecaption{\label{tab:pho}Multiwavelength photometry of two individual galaxies in MACS0647--JD (i.e., JDa and JDb). }
\tablewidth{\columnwidth}
\tablehead{
\colhead{Filter}&
\colhead{JD1a}&
\colhead{JD1b}&
\colhead{JD2a}&
\colhead{JD2b}&
\colhead{JD3a}&
\colhead{JD3b}
}
\startdata
F115W & $-18\pm3$ &  $-2\pm2$ & $-10\pm3$ & $-7\pm2$ & $-2\pm2$ & $-3\pm1$ \\
F150W & $144\pm3$ &  $27\pm2$ & $91\pm3$ & $16\pm2$ & $55\pm2$ & $7\pm1$ \\
F200W & $160\pm3$ &  $43\pm2$ & $115\pm2$ & $27\pm2$ & $60\pm2$ & $13\pm1$ \\
F277W & $143\pm2$ &  $37\pm2$ & $90\pm2$ & $27\pm1$ & $43\pm1$ & $8\pm1$\\
F356W & $106\pm2$ &  $39\pm1$ & $64\pm2$ & $25\pm1$ & $30\pm1$ & $9\pm1$\\
F444W & $97\pm3$ &  $44\pm2$ & $59\pm2$ & $26\pm1$ & $28\pm1$ & $8\pm1$ \\
F480M & $97\pm3$ &  $44\pm2$ & $59\pm2$ & $26\pm1$ & $28\pm1$ & $8\pm1$
%\vspace{-0.1in}
 \enddata
%\tablenotetext{a}{Observatory}
\tablenotetext{}{{\bf Note.} All fluxes are described in $\rm nJy$
and were measured using piXedfit \citep{Abdurrouf2021}.
}
%\red{All can be integers, without decimal points. Might add the stack total if there's room.
%For A \& B, I guess we'll provide for all 3 lensed images.
%Thinking about it more now, I think that ends up being a separate table, %especially if we present results from all methods.
%And we have those measurements in fewer filters, so it will be more compact.
%\tablenotetext{b}{1\sig\ point source sensitivity (nJy) within the same apertures}
\end{deluxetable*}
%\tablecomments{From http://www.stsci.edu/{\HST}/campaigns/frontier-fields/{\HST}-Survey}


==> properties_phot.tex <==
% Filters
\begin{deluxetable*}{lllccr}
\tablecaption{\label{tab:phy}Physical properties of MACS0647--JD estimated from \texttt{Bagpipes} corrected for magnification (flux ratio). }
%\tablecaption{\label{tab:phy}Photometric redshifts (\texttt{Bagpipes}) 
%and relative fluxes of JD1,2,3 used to normalize the magnification estimates.}
\tablewidth{\columnwidth}
\tablehead{
\colhead{}&
\colhead{JD1}&
\colhead{JD2}&
\colhead{JD3}&
\colhead{Combined}&
}
\startdata
Formation age ($\rm Myr$) &$160^{+69}_{-69}$& $151^{+60}_{-74}$ & $153^{+121}_{-75}$& $177^{+73}_{-71}$  \\
Mass-weighted age ($\rm Myr$) & $54^{+24}_{-23}$& $51^{+20}_{-25}$ & $51^{+43}_{-25}$& $59^{+25}_{-24}$  \\
Stellar Mass (${\rm log}(M_{*}/M_{\odot})$) & $8.62^{+0.11}_{-0.15}$ & $8.61^{+0.10}_{-0.18}$ &  $8.51^{+0.18}_{-0.22}$& $8.65^{+0.11}_{-0.14}$    \\
SFR ($M_\odot/{\rm yr}$) within 100 Myr &$4^{+1}_{-1}$& $4^{+1}_{-1}$ &  $3^{+1}_{-1}$&  $4^{+1}_{-1}$  \\
log sSFR (${\rm yr}^{-1}$) &$-7.98^{+0.05}_{-0.09}$ &$-7.96^{+0.04}_{-0.08}$ &  $-7.97^{+0.04}_{-0.16}$& $-8.00^{+0.07}_{-0.10}$ \\
Photometric Redshift &$10.64^{+0.06}_{-0.07}$ &$10.76^{+0.08}_{-0.09}$ & $10.50^{+0.14}_{-0.16}$  & $10.65^{+0.09}_{-0.10}$   \\
Relative flux ($\ge \rm F200W$) & 1 & 0.66 & 0.28 & 1.94\\
Magnification (flux ratio) & 8 & 5.3 & 2.2& 15.5 \\ 
{Magnification (lens model)} & 6.9 & 6.3 & 2.1 & 15.3 \\ 
%\vspace{-0.1in}
%Flux ratio ($\ge \rm F200W$) normalized to JD1 & 1 & 0.66 & 0.28 & 1.94\\
%Formation redshift &$14.8$&$14.7$& $14.3$ & $15.5$
{Tangential Magnification} & 4.7 & 4.4 & 1.8 \\
\enddata
\tablenotetext{}{
{{\textbf{Note}. 
%The systemic errors, including propagated errors from de-lensing, are not included in the error of estimated stellar masses and SFRs here, which will be another $\sim$ 8 per cent of uncertainty.
Magnification uncertainties are on the order of 15\% \citep{Meneghetti2017}
and are not included in the uncertainties quoted above for stellar mass and SFR.
}}}
%\tablenotetext{a}{Observatory}
%\tablecomments{\red{not sure whether to include physical parameter results}}
\end{deluxetable*}


==> scraps.tex <==

as an overdensity of red galaxies 
It was spectroscopically confirmed to be a cluster at redshift $z = 0.566$ by \cite{WenHan15}.


Discovered by Wen et al. (2012) based on photometric redshifts in SDSS-III. 
Renamed in the PSZ2 catalog with coordinates given in decimal degrees (Alternate Name above).

 the Wen, Han, & Liu SDSS-III cluster catalog (WHL; Wen et al. 2012);
 
 



The Planck survey 
This cluster was ranked as the 31st most massive cluster in the Planck PSZ2 catalog with a Sunyaev-Zeldovich calculated mass of $M_{500} = 9\times 10^{14} M_{\odot}$.

WHL J013719.8-082841 (henceforth \WHL) was discovered in SDSS imaging as an overdensity of red galaxies by \cite{WHL12}, and its redshift was subsequently confirmed at $z = 0.566$ by \cite{WenHan15}. 
This cluster was ranked as the 31st most massive cluster in the Planck PSZ2 catalog with a Sunyaev-Zeldovich calculated mass of $M_{500} = 9\times 10^{14} M_{\odot}$.  



\cite{Salmon2020} discovered at 15\arcsec\ long arc at $z_{phot} = 6.2$ lensed by this cluster and dubbed it the Sunrise Arc, prompting follow-up observations with HST (GO 15842, P.I. Coe). 
These follow-up images included 5 additional orbits of ACS F814W imaging, and two orbits each of ACS F475W and WFC3/IR F110W imaging, and are presented in detail in \cite{Welch2022_earendel}. 
The Sunrise Arc is shown in Figure \ref{fig:sunrise-arc}, and each of its 7 small clump structures are labeled. 
Additionally, this arc contains an extremely magnified lensed star presented in \cite{Welch2022_earendel}.
\WHL received a total of 7 hours of observations in the IRAC 3.6 $\mu$m band, and 5 hours in the 4.5$\mu$m band. 


The massive galaxy cluster 
WHL J013719.8-082841
(RA = 01:37:25.0,
Dec = $-$08:27:25.0,
$z = 0.566$)

$M_{500} = 8.9 \pm 0.7$

WHL J24.3324-8.477

WHL0137-08

later confirmed at $z = 0.566$ (Wen et al. 2015)

Within the Sunrise Arc, \citep{Welch22_Earendel} 
also discovered Earendel,
an individual star (or star system) at $z \sim 6$ magnified by a factor of thousands.
%the Sunrise Arc and Earendel lensed by \WHL.
%, the most highly magnified galaxy 


has the potential

Ancillary science includes discoveries of new distant lensed galaxies.

lensing higher redshifts
key to discovering the first galaxies with JWST

----------------------------

* JWST

* HST

* lensing magnification

* Sunrise Arc + Earendel

* WHL0137

* RELICS

* JWST 2282

* lensing most distant galaxies

----------------------------


The most spectacularly lensed galaxies were discovered in large ground-based surveys such as SDSS
or in follow-up imaging of galaxy clusters.


offers two advantages to complement ``blank field'' surveys.
First, the magnification reveals smaller spatial scales unattainable without a larger telescope.

Where blank fields revealed star forming clumps several 100 pc across,
lensed fields 
The kpc scale clumps observed in \HST\ images
gave way to lensed star clusters seves

in so many shapes, colors, and sizes, each galaxy unique with its own story to tell.

Galaxies evolved over cosmic time from small irregular clumpy clusters and chains
to majestic spirals and ellipticals we see at present day in the local universe.
Hubble looked 97\% of the way back to the Big Bang, seeing $z = 11$ galaxies as they were
13.4 billion years ago when the universe was just 400 million years old.
% Spitzer


The Hubble Space Telescope (HST) revealed the beautiful diversity of galaxies
in so many shapes, colors, and sizes, each galaxy unique with its own story to tell.
Galaxies evolved over cosmic time from small irregular clumpy clusters and chains
to majestic spirals and ellipticals we see at present day in the local universe.
Hubble looked 97\% of the way back to the Big Bang, seeing $z = 11$ galaxies as they were
13.4 billion years ago when the universe was just 400 million years old.
% Spitzer



offers the promise of efficiently discovering more distant galaxies (e.g., Coe+)
and magnifying distant galaxies to reveal small structures on parsec scales
that we couldn't see otherwise (Johnson, Vanzella, Welch).


The James Webb Space Telescope (JWST) is our generation's next great leap in technology
offering even deeper, higher resolution images extending to longer infrared wavelengths.
Every JWST image surpasses the Hubble Deep Fields, 
transforming our understanding of distant galaxies, revealing exquisite details
including tiny parsec scale star forming regions and low surface brightness tidal features,
and the full census of stellar mass in each galaxy 
including older and dustier populations invisible to Hubble too red and redshifted.


The correlation between R23 and metallicity is double-valued, shaped like an upside-down U
(see \citet{Nakajima2022} Figure 3),
but we can show the lower metallicity solutions are more likely.


Finally, we note Ne3O2 may be used to constrain metallicity,
though there is not a strong correlation.
In \cite{Nakajima2022},
the few galaxies with high Ne3O2 \about\ 2 
were clustered between roughly 5 and 13\% \Zsun
(7.4 $<$ \logOH\ $<$ 7.8).
%as similarly noted in \cite{Bunker2023}.

We detect the continuum between 1.3 and 5.3 \um\ with
SNR $>$ 10 per spectral resolution element out to \about 3\um,
with flux decreasing and noise increasing to longer wavelengths.

We detect the continuum between 1.3 and 5.3 \um,
rolling off to zero significant flux blueward of the Lyman break at 1.2 \um.
The continuum is detected with SNR $>$ 10 per spectral resolution element out to \about 3\um,
with flux decreasing and noise increasing to longer wavelengths.

The NIRSpec observations of MACS0647$-$JD were conducted as part of the \JWST\ Cycle 1 program GO 1433 (PI Coe).


NIRCam data came first in 2022 on September 23 in 6 filters, F115W, F150W, F200W, F277W, F365W, and F444W spanning 1--5$\,\mu$m, and the results were studied and presented in \citet{Hsiao2022}.
New \JWST\ NIRSpec data was obtained on January 8 and February 20.
The observing mode of NIRSpec observation is conducted in multi-object spectroscopy (MOS) mode.
Sources with interests are put in the slitlets, including JD1A, JD2, JD3, and JDC.
Total exposure time is XXX and XXX for each observation.
A zoomed-in view of slitlets is shown in Figure \ref{fig:slitlets}.

We process all \JWST\ and \HST\ images with grizli, 
drizzled to a common pixel grid
with coordinates registered to GAIA DR3 \citep{Gaia_EDR3}.


\section{Conclusions}
\label{sec:conclusions}
In this study, we report NIRSpec observations of MACS0647$–$JD obtained as part of the same JWST observation program GO 1433 (PI Coe).
We detect 6 emission lines with SNR$>5$, including \CIIIdw, \OIIw, \NeIIIw, \NeIIIwb, \Hdelta, and \Hgamma\ and two marginal detections with SNR of 4.4 and 2.8 for \OIIIwa\ and \HeI, respectively.
Based on the observed wavelengths of these emission lines,
we measure the spectroscopy redshift $z=10.17$.
%We measure the redshift to be $z=10.17$ based on the emission lines.

Some of the most useful lines to study the star-formation rates, the ionization parameter, and metallicity, including \Halpha, \Hbeta, and \OIIIw\ are 
redshifted beyond the wavelength coverage of NIRSpec for MACS0647$-$JD at $z=10.17$.
The line ratio \NeIII/\OII\ can still be a useful diagnostic for ionization parameter log(U) and can also help constrain gas-phase metallicity Z.
We estimate the ionization parameter of ${\rm log(U)}=-1.8\pm0.2$, and the log(U) from SED fitting is slightly higher, which is ${\rm log(U)}=-1$.
We also detect both \Hdelta\ and \Hgamma.
The line ratio of ${\rm H}\delta/{\rm H}\gamma=1.88\pm0.43$, which is consistent with 1.81 expected for Case B recombination at $T\sim10000\,K$.
Assuming no dust, we estimate the strength of \Halpha\ and estimate SFR$=1.4\pm0.2\,M_{\odot}/{\rm yr}$, which is similar with the SFR from SED fitting and SFR inferred from \OII\ (${\rm  SFR_{OII}}=0.7\pm0.2\,M_{\odot}/{\rm yr}$).
We adopt various ways to reach metallicity, including Ne3O2, O32, and R23 (the last two ratios are estimated from Ne3O2), suggesting a metallicity of $Z=0.2\pm0.1\,Z_{\odot}$.

\OIII, \Halpha, and \Hbeta\ will fall in the wavelegnth regime in \JWST\ MIRI, which is predicted to be detected based on the estimated star-formation rate.
Possible future observation will give us more direct measurement of the line ratios to estimate physical properties of interest such as star-formation rates, metallicity, and the dust. 

We detect 6 emission lines with SNR$>5$, including \CIIIdw, \OIIw, \NeIIIw, \NeIIIwb, \Hdelta, and \Hgamma\ and two marginal detections with SNR of 4.4 and 2.8 for \OIIIwa\ and \HeI, respectively.

Some of the most useful lines to study the star-formation rates, the ionization parameter, and metallicity, including \Halpha, \Hbeta, and \OIIIw\ are 
redshifted beyond the wavelength coverage of NIRSpec for MACS0647$-$JD at $z=10.17$.
The line ratio \NeIII/\OII\ can still be a useful diagnostic for ionization parameter log(U) and can also help constrain gas-phase metallicity Z.
We estimate the ionization parameter of ${\rm log(U)}=-1.8\pm0.2$, and the log(U) from SED fitting is slightly higher, which is ${\rm log(U)}=-1$.
We also detect both \Hdelta\ and \Hgamma.
The line ratio of ${\rm H}\delta/{\rm H}\gamma=1.88\pm0.43$, which is consistent with 1.81 expected for Case B recombination at $T\sim10000\,K$.
Assuming no dust, we estimate the strength of \Halpha\ and estimate SFR$=1.4\pm0.2\,M_{\odot}/{\rm yr}$, which is similar with the SFR from SED fitting and SFR inferred from \OII\ (${\rm  SFR_{OII}}=0.7\pm0.2\,M_{\odot}/{\rm yr}$).
We adopt various ways to reach metallicity, including Ne3O2, O32, and R23 (the last two ratios are estimated from Ne3O2), suggesting a metallicity of $Z=0.2\pm0.1\,Z_{\odot}$.

\OIII, \Halpha, and \Hbeta\ will fall in the wavelegnth regime in \JWST\ MIRI, which is predicted to be detected based on the estimated star-formation rate.
Possible future observation will give us more direct measurement of the line ratios to estimate physical properties of interest such as star-formation rates, metallicity, and the dust. 

%\subsection{Prospects of future JWST observations}
Merge with text above:

In this study, since \Halpha, \Hbeta, \OIIIw, are beyond the coverage of NIRSpec, we mostly use Ne3O2 to estimate other line ratios, metallicity, and the ionization parameter.
However, the other line ratios we derive, such as O32 and R23, are indirect.
Therefore, detecting these lines is awaited to infer the star-formation rates, metallicity, and dust more directly.
These lines fall in the JWST MIRI wavelength regime.
Possible future JWST MIRI observations may help to understand the physical conditions of MACS0647$-$JD and the universe beyond the redshift of $z=10$ in more detail. 


-----

%especially at high values Ne3O2 $> 1$
%in star forming galaxies at $z = 0 - 7$
%\citepeg{Jaskot2013, Izotov2018, Witstok2021, Flury2022, Tang2023}.

The line ratio Ne3O2 $=$ \NeIIIw\ $/$ \OIIw\ is a useful diagnostic for ionization parameter \logU\ and can also help constrain gas-phase metallicity $Z$ \citepeg{Levesque2010,Witstok2021}.
%Galaxies with \NeIII\ stronger than \OII\ have high ionization parameters and low metallicities.
In MACS0647-JD, we find \NeIII\ is stronger than \OII\ in all four observations.
In the stacked spectrum, we measure Ne3O2 $= 1.8 \pm 0.2$.
This corresponds to \logU\ $= -1.84 \pm 0.06$ 
based on a tight relation from \citet[][Equation 3]{Witstok2021}:
\logU\ $=0.884\times\rm{log(Ne3O2)}-2.07$.

The line ratio Ne3O2 is strongly correlated with 
the line ratio O32 $=$ \OIIIww\ $/$ \OIIw\ and is used more commonly 
because \OIII\ and \OII\ are usually both stronger than \NeIII.
In our case, \OIII\ is redshifted beyond our wavelength coverage.
%so we turn to \NeIII\ and the Ne3O2 ratio, which has one advantage: 
%being insensitive to dust since \NeIII\ and \OII\ are at similar wavelengths.
%based on strong correlations at these high values
%observed in star forming galaxies at $z = 0 - 7$
Correlations between Ne3O2 and O32 are especially strong at high values Ne3O2 $> 1$
in star forming galaxies at $z = 0 - 7$
\citepeg{Jaskot2013, Izotov2018, Witstok2021, Flury2022, Tang2023}.

Based on the ratio Ne3O2 $=1.8\pm0.2$, we estimate O32 $\sim 30 \pm 0.2$ dex.
% Flury2022: LzLCS z ~ 0.2 - 0.4
% local LyC leakers Witstok2021: we will consider a sample compiled from Izotov et al. (2016a,b, 2018a,b), Gazagnes et al. (2020), and Guseva et al. (2020), together simply the ‘Izotov et al. sample’
% Jaskot & Oey 2013: z ~ 0 green peas
% Tang2023: z > 7
%
Given this estimate for O32 and our observed line flux for \OII, 
we can estimate the expected \OIIIw\ line flux 
\about\ \tentotheminus{17} \cgsfluxunits.
%(redshifted beyond our wavelength coverage).
%$3 \times$
Note the \OIIIw\ line is 2.98 times stronger than \OIIIwc\ \citep{StoreyZeippen2000},
so our estimated combined \OIIIww\ flux is 1.34 times the \OIIIw\ flux.

We first model the \JD\ total photometry measured in the NIRCam images
by \grizli\ for lensed image JD1 with a magnification $\mu = 8 \pm 1$.
We exclude the F150W photometry because our spectral models do not include Lyman damping.
(Including the F150W photometry results in artificially low ages $< 2$ Myr.)

** Rewrite the rest of this section, referring to results in the new Table \ref{tab:indi_phy} rather than writing them out here.

First assuming a constant SFR, we measure young formation ages $16^{+16}_{-9}$ Myr.
The mass-weighted ages are half those values: $8^{+8}_{-5}$ Myr.
We measure a delensed SFR $10 \pm 3$ \Msun\ yr\inv\ and stellar mass \logM\ $= 8.1 \pm 0.3$,
including both modeling and lensing uncertainties.
The specific SFR (sSFR $\equiv$ SFR / stellar mass) is ...
log(sSFR / Gyr\inv) = $-7.1 \pm 0.3$ if using the current SFR
...
or log(sSFR / Gyr\inv) = $-8$ by definition if averaging over 100 Myr? 
Let's average over 10 Myr...
***
%or log(sSFR) $= -8.0 \pm 0.3$, consistent with that estimated in \cite{Hsiao2022}.


We find similar results with a ``delayed $\tau$'' star formation history 
that allows for a linear rise followed by an exponential decline:
SFR($t$) $\propto t\, \exp(-t / \tau)$.
Most of our fits only have the linear rise with $\tau > 1$ Gyr.
%
Finally, we explore non-parametric star formation histories
with constant SFR in 4 time bins (e.g., 0 -- 10 -- 50 -- 150 -- 300 Myr).
Regardless of the time bins we choose, we never find significant SFR in any older populations.


Next, we model the clump A photometry measured by \piXedfit\ in JD1A magnified by $\mu = 8 \pm 1$.
Constant star formation models again yield young formation ages $17^{+5}_{-4}$ Myr
with mass-weighted ages $8^{+3}_{-2}$ Myr,
delensed SFR of $3 \pm 1$ \Msun\ yr\inv\ and stellar mass \logM\ $= 7.6 \pm 0.2$,
and very little dust $A_V < 0.01$ mag.
Other star formation histories yield similar results.
These age estimates are towards the low end of those (1 -- 50 Myr) presented in \cite{Hsiao2022} for clump A.

The smaller redder component B photometry is best fit by a linearly rising SFR for 40 -- 300 Myr,
with a mass-weighted age 10 -- 110 Myr,
stellar mass \logM\ $= 7.7^{+0.2}_{-0.3}$,
and dust $A_V = 0.13 \pm 0.07$ mag.
Based on similar age estimates in \cite{Hsiao2022},
they suggested clump B may have formed separately and merged with the younger clump A,
though different star formation histories in situ are also possible.




We present JWST/NIRSpec prism spectroscopy of MACS0647-JD, the triply-lensed $z \sim 11$ candidate discovered in HST imaging and spatially resolved by JWST imaging into two components A and B.
Spectroscopy of component A yields a spectroscopic redshift $z=10.17$ 
based on 7 detected emission lines:
C\,{\sc iii}]\,$\lambda\lambda$1907,1909,
[O\,{\sc ii}]\,$\lambda$3727,
[Ne\,{\sc iii}]\,$\lambda$3869,
[Ne\,{\sc iii}]\,$\lambda$3968,
H$\delta$\,$\lambda$4101,
H$\gamma$\,$\lambda$4340,
and [O\,{\sc iii}]\,$\lambda$4363.
These are the second-most distant detections of these emission lines to date, 
in a galaxy observed just 460 million years after the Big Bang. 
Based on observed and extrapolated line flux ratios
we derive a gas-phase metallicity $Z =$ \logOH\ = 7.5 -- 8.0, or (0.06 -- 0.2) $Z_\odot$,
ionization parameter log($U$) $\sim -1.9\pm0.2$,
and an ionizing photon production efficiency 
${\rm log}(\xi_{\rm ion})=25.2\pm0.2\,$erg$^{-1}$ Hz.
The spectrum has a softened Lyman-$\alpha$ break,
evidence for a strong Ly$\alpha$ damping wing,
suggesting that MACS0647-JD was unable to ionize its surroundings
beyond its immediate vicinity ($R_{\text{HII}} \ll 1$ pMpc).
The Ly$\alpha$ damping wing also suppresses the F150W photometry,
explaining the slightly overestimated photometric redshift $z = 10.6 \pm 0.3$.
MACS0647-JD has a stellar mass log($M/M_\odot$) = $8.1 \pm 0.3$,
including $\sim$ 6$\times 10^7 M_\odot$ in component A,
most of which formed recently (within \about 20 Myr)
with a star formation rate $2\pm1 M_\odot$ / yr, all
within an effective radius $70\pm24\,$pc.
The smaller component B ($r \sim 20$) pc
is likely older ($\sim$100 Myr) with more dust ($A_V \sim 0.1$ mag),
as found previously.
Spectroscopy of a fainter companion galaxy C separated by a distance of \about\ 3$\,$kpc 
reveals a Lyman break consistent with $z = 10.17$.
MACS0647-JD is likely the most distant galaxy merger known.

